Neural Contextual Bandits without Regret

Contextual bandits are a rich model for sequential decision making given side information, with important applications, e.g., in recommender systems. We propose novel algorithms for contextual bandits harnessing neural networks to approximate the unknown reward function. We resolve the open problem of proving sublinear regret bounds in this setting for general context sequences, considering both fully-connected and convolutional networks. To this end, we first analyze NTK-UCB, a kernelized bandit optimization algorithm employing the Neural Tangent Kernel (NTK), and bound its regret in terms of the NTK maximum information gain $\gamma_T$, a complexity parameter capturing the difficulty of learning. Our bounds on $\gamma_T$ for the NTK may be of independent interest. We then introduce our neural network based algorithm NN-UCB, and show that its regret closely tracks that of NTK-UCB. Under broad non-parametric assumptions about the reward function, our approach converges to the optimal policy at a $\tilde{\mathcal{O}}(T^{-1/2d})$ rate, where $d$ is the dimension of the context.

==> Old Versions/outline.tex <==
\section{Outline}

\begin{enumerate}
    \item \textbf{Introduction}
    \begin{itemize}
        \item Motivate
        {\small \color{airforceblue} 
        \begin{itemize}
            \item[--] We want bandit optimization algorithms that substitute the GP/Kernel regression module with NN GD training. 
            \item[--] But why? Expressiveness and convenient computation? 
            \item[--] Should I particularly mention applications of CNNs and bandits?
            \item[--] Should I separately motivate NTKs? Or the story is that our main goal is the Approximate algorithm and \textsc{NTK-UCB} is just a bridge?
        \end{itemize}}
        \item What we do (High-level)
        {\small \color{airforceblue}
        \begin{itemize}
            \item[--] 1-2 sentence intro to the algorithm. Will have to mention \textsc{GP-UCB} without having introduced it...
            \item[--] We present a technique (?) for giving sublinear regret bounds on these (C)NN-based algorithms, via the information gain.
            \item[--] Using this pipleline We give bounds for a deep fc NN, and a 2-layer CNN.
        \end{itemize} }
        \item Related Work
                {\small \color{airforceblue}
        \begin{itemize}
            \item[--] NTK works: ones that introduce them and ones that give properties. GD on NN at infinite width. Work on CNTKs and rotation invariant kernels.
             \item[--] Info gain bounds.
            \item[--] UCB Regret bounds. Elaborate on Neural-UCB.
        \end{itemize}}
        \item Summary of Results
        {\color{airforceblue}
        \begin{itemize}
            \item[--] First to give Info gain bound for Deep NTKs and two-layer CNTKs. We show a $\mathcal{O}(\sqrt{T})$ rate for both, however the coefficient is reduced by a factor of $d$ for the CNTK.
            \item[--] We introduce the NTK-UCB. We bound its regret under GP and RKHS assumptions. We show that same bound holds for the CNTK-UCB, the convolutional counterpart. 
            \item[--] We use NTK-UCB as an intermediate step towards the NN-UCB, which trains a NN as a substitute for performing posterior mean with the NTK. 
            \item[--] We are the first to give a sublinear regret bound for an NN-based bandit optimization method. We show that if the width of the incorporated network in NN-UCB is large enough (poly rate with $T$), then the $\mathcal{O}(T^{3/4})$ regret guarantee holds for NN-UCB, under RKHS assumption.
            \item[--] We introduce the CNN-UCB as a variant of the NN-UCB, by swapping the deep NN with a 2-layer CNN. We show that in the infinite width limit, the regret for CNN-UCB is sublinear. Same rate, coef reduced by $d$.
            
        \end{itemize}}
        \item Outline of the Paper
        {\small \color{airforceblue} If enough space}

    \end{itemize}
    \item \textbf{Background and Problem Statement}
    
    \begin{itemize}
     \item Problem Statement
     \iffalse
        {\small \color{airforceblue}
        \begin{itemize}
            \item[--] Just the $y = f(\vx) + \epsilon$ model, def of $R_T$, finite number of actions, $\mathcal{X} \subset \sS^{d-1}$. 
            \item[--]  goal $R_T/T \rightarrow 0$ as $T \rightarrow \infty$ under some assumption on true reward $f$
        \end{itemize}}
        \fi
    \item GP and RKHS Assumption
    \iffalse
        {\small \color{airforceblue}
        \begin{itemize}
             \item[--] Assumptions on $f$ and $\mathcal{X}$. Explain how neither GP nor RKHS assumption contains the other.
             \item[--] Maybe motivate why the assumptions are broad.
             \item[--] How much detail should I give here? Should I talk about what it means for $f$ to be a member of $\mathcal{H}_k$?
             \item[--] Should I mention here that \textsc{GP-UCB}'s regret as an example?
        \end{itemize}}
        \fi
            \item Neural Tangent Kernels
            \iffalse
        {\small \color{airforceblue}
        \begin{itemize}
        \item[--] Formally define a neural network.
            \item[--] NTK: Where it comes from, mercer decomposition, its RKHS.
            \item[--] Forward reference to CNTK section.
            \item[--] Discussion on eigendecay of the NTK? or do I leave it for the infogain section?
           
        \end{itemize}}
 \fi
    \end{itemize}
    \item \textbf{NTK-UCB}
    \begin{itemize}
        \item Intro.
        \iffalse
            {\small \color{airforceblue}
            \begin{itemize}
                \item[--] This algorithm is an intermediate step...?
            \item[--] Should I separately talk about GP optimization before going into GP-UCB? Mentioning that posterior mean function has a bounded kernel norm would be insightful.
            \item[--] Policy
                \item[--] NTK-UCB is just GP-UCB, with the NTK kernel as the covariance function. Should I give the algorithm too?
                \end{itemize}}
                \fi
        \item Information Gain
\iffalse
        {\small \color{airforceblue}
                \begin{itemize}
        \item[--] Open with GP-UCB: Info gain quantifies speed of learning
        \item[--] Define and give expression under our setting $\log (\mI+ \sigma^{-2}K)$
        \item[--] How it appears in regret bounds and that it has to be at least sublinear with $T$.
        \item[--] The bound
        \item[--] Maybe a history of info gain bounds for Mat\'ern kernels? We extend previous literature to include $\nu = 0.5$ case.
        \item[--] Applications and Implications of the theorem
        \item[--] Proof sketch. We use Mercer property of the NTK.
        \end{itemize}}
        \fi
         \item GP Regret.
         \iffalse
            {\small \color{airforceblue}
            \begin{itemize}
                \item[--] Regret under GP Thm
                \item[--] Give cor of the form $\tilde{\mathcal{O}}(C(d, L)T^{3/4})$ by plugging in info gain Thm.
                \item[--] One liner proof sketch.
                                \end{itemize}}
                                \fi
         \item RKHS Regret.
         \iffalse
            {\small \color{airforceblue}
            \begin{itemize}
                 \item[--] Using this proof sketch, give intuition on why RKHS assumption has additional challenges, specially when we have NTKs.
                 \item[--] To overcome this issue, we bound the regret for the sup variant.
                 \item[--] Give sup algorithm pseudo code
                 \item[--] Give 1-2 sentence explanation on why it helps. Refer details to appendix.
                \item[--] Regret under RKHS Thm
                \end{itemize}}
                \fi
    \end{itemize}
     \item \textbf{NN Regret Bound}
        \begin{itemize}
            \item Intro
            \iffalse
            {\small \color{airforceblue}
            \begin{itemize}
            \item[--]We are now ready to introduce the NN-UCB. It swaps Bayesian Inference with NN training. It results from approximating the posterior mean and variance in NTK-UCB, via properties of the NTK.
            \item[--] Approximating $\mu^{(\text{post})}$.
            \item[--] Approximating $\sigma^{(\text{post})}$.
            \item[--] Full algorithm (give pseudo code)
            \item[--] Give big picture: NN-UCB is similar to performing GP-UCB with a random feature model. Where the features are elements of the gradient of a network at initialization.  
            \item[--] Give big picture alternative: Compare $\mu^{(\text{post})}$ and $f^{(\text{GD})}$ by talking about their corresponding loss functions.
                        \begin{align*}
                                \Ls_0(\vtheta) &= \sum_{i\leq t} (\bm\phi^T(\vx_i)\vtheta - y_i)^2 + \sigma^2\norm{\vtheta}_2^2\\
                                \Ls_1(\vtheta) & = \sum_{i\leq t} (\vg^T(\vx_i; \vtheta^{(0)})\vtheta - y_i)^2 + m\sigma^2\norm{\vtheta}_2^2\\
                                    \Ls_2(\vtheta) & =  \sum_{i\leq t} (f(\vx_i;\vtheta) - y_i)^2 + m\sigma^2\norm{\vtheta-\vtheta^0}_2^2
                        \end{align*}
                         \end{itemize}}
                         \fi
            \item Regret Bound
            \iffalse
            {\small \color{airforceblue}
            \begin{itemize}
            \item[--] First give additional assumptions needed for this theorem
            \item[--] Lemma: For i.i.d samples, if network is wide enough, solution of GD on Regularized Loss is close to the posterior mean of GP with NTK and noisy observations.
            \item[--] Alternative: For i.i.d noisy samples and under RKHS assumption, if the network is wide enough, solution of GD on Regularized Loss is close to the true reward.
            \item[--] Similar challenge as in NTK-UCB with RKHS assumption. We prove the regret for the sup variant.
            \item[--] Give Sup variant pseudo code
            \item[--] NN-UCB Regret Thm 4
            \item[--] Parameter dependency, explain the terms in bound, proof idea and how its related to proof of Thm 3.
            \item[--] Corollary after plugging in information gain 
            \item[--] Comparison with Neural-UCB.
        \end{itemize}}
        \fi
        \end{itemize}
    \item \textbf{CNN Extensions}
    \begin{itemize}
    \item Bridge from NN to CNN, NTK to CNTK.
        {\small \color{airforceblue}
        \begin{itemize}
            \item[--] Define CNN as $\mathcal{G}_d$ invariant NN, i.e., NN averaged over all circular shifts of the input
            \item[--] Lemma (from \citet{mei2021learning}): CNTK is also the NTK averaged over all circ-shifts of \textit{one} input (due to rotation invariance at infinite width)
            \item[--] Optional: intuition/proof for lemma, via first order approximation of the CNN vs first order approximation of the NN.
            \item[--] Theorem/lemma: CNTK's Mercer decomposition. Algebraic Multiplicity is reduced by a factor of $d$.
            \item[--] Optional: Intuition via Degeneracy number of $\mathcal{G}_d$.
        \end{itemize}}
    \item CNTK bounds
        {\small \color{airforceblue}
        \begin{itemize}
            \item[--] Thm: Infogain bound for the CNTK.
            \item[--] Compared to infogain for NTK, we learn $d$ times faster about the underlying function.
        \item[--] Regret bound: Thm 2 and Thm 3 hold for the CNTK.
        \end{itemize}}
    \item CNN-UCB Regret Bound
        {\small \color{airforceblue}
        \begin{itemize}
            \item[--] Lemma: $\bar \vg^T(\vx)\bar\vg(\vx')$ converges to $\bar k(\vx, \vx')$ as $m \rightarrow \infty$. 
            \item[--] Lemma: $\bar f^{(\text{GD})}$ converges to $\hat{\bar \mu}$ if $m$ is large enough (polynomial rate with $T$).
            {\color{amaranth} \item[--] We have some lemmas showing that for a 2-layer CNN with large enough width, running GD doesn't change the gradient vector and the parameters. These are new, but simple extension from existing NN results. Should I mention in main text?}
            \item[--] At $m \rightarrow \infty$, with other conditions unchanged, Thm 4 holds for CNN-UCB.
            {\color{amaranth}
            \item[--] Alternative: I might be able to show that for polynomial $m$, Thm4 roughly holds for CNN-UCB, with $ R_T = \mathcal{O}(\sqrt{T\hat{\bar\gamma}_T})$. Here $\hat{\bar\gamma}_T$ is the information gain when we're using the empirical gram matrix of the CNN as the kernel matrix. }
            \item[--] Cor: At $m \rightarrow \infty$, CNN-UCB is sublinear with $\mathcal{O}(\frac{C(d,L)}{d} T^{3/4})$.
            \item[--] Conclude that convolutional variants are potentially faster for larger $d$s, while they have the same rate with $T$.
        \end{itemize}}
    \end{itemize}
    \item \textbf{Experiments}
    \begin{itemize}
        {\color{airforceblue} \item Strongly depends on how much space is left.} 
    \end{itemize}
    \item \textbf{Conclusion}
    \begin{itemize}
        \item Quick recap of what we did.
        \iffalse
        \item Concrete Questions
                {\small \color{airforceblue}
        \begin{itemize}
        \item[--] We prove new result on GD with 2-layer simple CNN, and the eigen decay of the 2-layer CNN. What about Extension to deeper CNNs?
        \item[--] Non-assymptotic CNN-UCB Regret
        \item[--] Optional: Further Connections of Bayesian optimization and NN Training? (Vague, form better)
        \item[--] Optional: Effects of finite width limit: I makes the kernel rotation invariant. Does it reduce approximation power?
        \item[--] What else?
        \end{itemize}}
        \fi
    \end{itemize}
\end{enumerate}

